Brickify: Enabling Expressive Design Intent Specification through Direct Manipulation on Design Tokens

Expressing design intent using natural language prompts requires designers to verbalize the ambiguous visual details concisely, which can be challenging or even impossible. To address this, we introduce Brickify, a visual-centric interaction paradigm -- expressing design intent through direct manipulation on design tokens. Brickify extracts visual elements (e.g., subject, style, and color) from reference images and converts them into interactive and reusable design tokens that can be directly manipulated (e.g., resize, group, link, etc.) to form the visual lexicon. The lexicon reflects users' intent for both what visual elements are desired and how to construct them into a whole. We developed Brickify to demonstrate how AI models can interpret and execute the visual lexicon through an end-to-end pipeline. In a user study, experienced designers found Brickify more efficient and intuitive than text-based prompts, allowing them to describe visual details, explore alternatives, and refine complex designs with greater ease and control.

==> texfiles/1-introduction-old.tex <==
\section{Introduction}
% \outline{
% P1: \\
% 1) popularity of using GenAI tools to generate graphic designs: Dalle, MidJourney, Adobe Firefly, etc; \\
% 2) current progress on GenAI research: performance improvement, direct manipulation interface (DirectGPT), node-graph editor for ideation, prompt expansion, etc. \\

% P2 (maybe separate into two paragraphs):\\
% However, leveraging GenAI to create graphic designs remains challenging for professional designers. \\
% 1) writing detailed textual instructions (prompts) is hard;
% the style, by nature, is ambiguous to find concrete and precise textual words to express, instead, it usually comes from visual inspirations like Pinterest, and could be a combination of several existing styles; \\
% 2) user-expressed style in their mind could be misaligned with what is interpreted by the models; \\
% 3) unclear design plans until several iterations. However, controllable iterations on design attempts are hard to achieve: 
% a) hard to use natural language to precisely select the object of interest in the design; 
% b) limited to the model capability, cannot isolate a certain object to refine without influencing others; 
% \\

% P3 (Research Questions): \\
% RQ1: How to allow users to better express their intentions regarding styles? \\
% RQ2: How to ensure their expressed intention is correctly conceived by GenAI models and enable the iterative controllable design iterations? \\

% P4: \\
% What we propose in this paper: 
% 1) use the mood board as a complementary to the textual prompt. 
% Textual prompt for ``factual'' instructions while mood board is more feasible to express vague ``style'' intentions. 
% However, the mood board usually contains many visual inspirations, thus leading to a huge possible design space, which can cause misinterpretation and misaligned generated results. 
% 2) Thus, we adopted the progressive editing way to allow users to check and modify in each step, largely narrowing down the design space, and thus, the controllability can be guaranteed. 
% \\

% P5 (Contributions): \\
% 1) a formative study and a content analysis to understand:
% a) how designers use the mood board; 
% b) the challenges in using current prompt-based GenAI tools; 
% c) how they iterate and refine the generated designs using the current tools and what's the challenges. \\
% 2) an interactive system to support visual prompting and progressive edits; \\
% 3) user study findings.
% }

Recent generative AI applications, such as \textit{MidJourney}, \textit{DreamStudio}, and \textit{DaLLE}, have demonstrated remarkable capabilities in producing graphic designs with human-level fidelity. 
\ryan{Add references for MidJourney, DreamStudio, and DaLLE.}
These tools have become invaluable for improving designers' productivity, aiding in brainstorming, quick prototyping, and inspiring new design possibilities through their generative variability. 
Different from the traditional WIMP interfaces of design editors, they introduce a new interaction paradigm working in an end-to-end fashion: a natural language prompt goes in and an image comes out, with little chance to intervene in between. 
Such prompt-driven interaction is recognized as \textit{intent-based outcome specification} by Neilson~\etal~\footnote{https://www.nngroup.com/articles/ai-paradigm/} where users no longer tell the system \textit{what to do} but \textit{what outcomes they want}.

Despite such an interaction paradigm reducing users' manual efforts to implement every detail in their minds, it presents unique challenges in the field of design: 
(i) the intent itself can be ambiguous to verbalize due to the disparity between written and visual languages.
\ryan{intent may be confusing to use here, not sure. I think many folks think of intents as very broad classes, especially in the co-pilot/AI assistant side of things, where an intent could actually be simply generating an image from text. In NLP, there is an area called intent classification which is big. Maybe we can change intent to goal, or something a bit more personal/specific. Again, I don't feel strongly about this, just pointing out potential confusion that might arise from intent terminology.}
Most research efforts have focused on enhancing the textual description aspect through prompt engineering~\cite{}, with some efforts like DirectGPT~\cite{masson2023directgpt} and PromptPaint~\cite{chung2023promptpaint} introducing visual metaphors for more direct manipulation. 
However, the primary reliance on textual prompts does not fully address the mismatch between the \textit{textual-centric} interaction mode and the \textit{visual-centric} thinking inherent in design practices;
(ii) the alignment between the specified intent and the generated outcome cannot be guaranteed due to the unaddressed issue of insufficient \textit{prompt-following}~\cite{betker2023improving} capabilities in foundation models, and the partial misalignments are hard to fix while keeping the rest intact due to the entanglement problem~\cite{}; 
(iii) the outcomes are presented as complete wholes without allowing for iterative refinement or flexible re-composition due to there being no turn-taking and gradual progress. 
Spellburst~\cite{angert2023spellburst} have explored branching and versioning with node-based interfaces but failed to decompose the outcome;
PromptPaint~\cite{chung2023promptpaint} has exploited the in-painting and out-painting for modular generation which typically require users to specify the regions by drawing masks in an image where details should be added or modified. 
While helpful in object decomposition, it falls short in separating styles, colors, and other design elements, leading to a constrained exploration space.
Together, the above-mentioned challenges make this \textit{outcome-oriented} interaction paradigm fail the existing \textit{process-oriented} mental model employed by graphic designers when seeking creative possibilities.

Reflecting on the traditional design practices, they align closely with the \textit{Geneplore} cognitive model~\cite{finke1996creative}, 
which delineates the creative process into \textit{generative} and \textit{exploratory} processes.
Designers often start with creating the mood board, a collection of images, shapes, swatches, colors, textures, and other visual stimuli, as an aid for conducting visual research, namely, framing, aligning, paradoxing, abstracting, and directing the design~\cite{lucero2012framing}. 
This stage corresponds to the \textit{generative process} of the \textit{Geneplore} model, and the produced mood board is termed as \textit{preinventive structures}. 
These structures are intentionally ambiguous, allowing for several ways of interpretation, and are central to probing the exploration of creative possibilities. 
Following this, designers engage in the process of interpreting the mood board on both abstract (\eg, style, atmosphere, mood) and concrete (\eg, elements to reuse) levels, methodically integrating diverse visual elements to forge a cohesive design with the bottom-up manner. 
This iterative process of refinement and decision-making is the typical \textit{exploratory process} of the \textit{Geneplore} model. 
Here, design efforts are carried out in an organized and controllable way, using local and serial processing to deliberately navigate the creative landscape, for example, separating individual design units with different layers, strategically comparing different combinations, and organizing histories. 


Comparing the way designers interact with the generative models with their traditional workflow, both the \textit{generative} and \textit{exploratory} processes in \textit{Geneplore} model are inadequately supported.
First, the \textit{generative process} is completely missing, and the \textit{preintentive structures}, \ie, visual stimuli, are replaced with textual prompts which emphasize clarity, descriptiveness, and precision but lack generative depth for encouraging exploration and reinterpretation.
Moreover, the \textit{exploratory process} is simplified to selecting one outcome from several (typically four) offered candidates whose variances are random, and the series of design decisions and the experimentation trajectory are disappeared.

To bridge the gap between designers' mental model and the prompt-driven interactions, we introduce a new paradigm: interacting with the generative models through both \textit{visual} and \textit{textual} prompts in a \textit{progressive editing manner}.
In specific, we bring the mood board back to the generative workflow, using such visual language as a complementary to the textual prompt: textual prompt serves for \textit{factual} instructions while the mood board for expressing ambiguous \textit{style} intents.
Furthermore, we explored the progressive editing manner to decompose the generation process into a series of design units and allow users to check and modify each step.
By doing so, we aim to minimize the misalignment and maximize the controllability.
Additionally, we organize the design journey into a composable node-based graph for further exploration.
We implemented the system of \sysname{} as a test-bed. 
We evaluated how \sysname{} impacts designers' creative experience with \x designers with different levels of expertise in a controlled in-lab user study. 
Participants found \sysname{} enabled a more intuitive intent-expressing way and provided an overall more diverse, fluid, and engaging experimentation experience. 
This research thus has the following contributions:
\begin{itemize}
    \item A formative study, to understand users' needs and frustrations on using the current prompt-based AI generation system; and how mood boards are created, utilized, and interpreted during the design process;
    \item A content analysis, to distill the common design units during the design processes;
    \item A prototype system, \sysname{}.
    \item A user study.
\end{itemize}




==> texfiles/design_insights_removed.tex <==
\subsection{Design Insights}
Our design decisions are shaped by insights gathered during the iterative design process ($S_{1-3}$) and grounded in existing literature. 
We articulate the following key design insights (\textbf{$D_{s}$}) behind our core concept of \emph{interactive design tokens}. 

\subsubsection{\textbf{D1: Interactive design tokens as the visual thinking tool and communicative medium between designers and AI models.}}

1. help designers to mark their attended primitive parts --- support designers' visual thinking;
2. help designers to tell AI what they have attended --- support communication between users and AI about what they have attended because AI isn't trained as designers to have that active vision;
3. help designers to tell AI how they plan to construct the attended elements --- support users control over the design. 
overall, mediating the information parsing among images, designers, and AI.

supporting visual-centric interaction paradigm, also closely entangled with supporting designers' natural visual thinking process.
visual thinking tool --- reflect the challenge 1- Inconvenience to organize references; 
communicative medium --- mediating communication between designers and AI. solve change 2 - hard to verbalize intent


\textbf{D1.1: Supporting designers' visual thinking process.}
Our interview study (S1) revealed that designers would organize and annotate reference images as part of their visual research, focusing on specific elements rather than the entire image. 
This selective focus, known as \emph{active vision}, is a crucial aspect of \emph{visual thinking}, which has been widely studied in cognitive science literature. 
Given the limitations of human working memory, externalizing these attended elements through annotations or organization is important --- these externalizations are called \emph{the extended mind}.
However, current generative AI tools fail to support this visual thinking process, as noted in C1 where designers are forced to rely solely on internal thought.
We argue that it is necessary to have the external \emph{objects of thought} inserted into the current workflow to reduce designers' cognitive load and thereby support a more efficient design process.


\textbf{D1.2: Mediating the communications between designers and AI.}
--- what and how
--- separation of what and how

Designers have the \emph{active vision} while AI models not, or at lease, not fully align with designers' visions.
Thus it is important for designers to clearly tell AI \emph{what} primitive elements they have attended, but often, referring them with natural language is difficult (C2). 
Additionally, 

C3 - how - telling AI about their active vision and how to use them. 
These communicative failures inspire us to propose the solution of adding a mediator to bridge such a mismatch.

Additionally, the separation of specifying what and how --- what information and design concepts to parse reflects on the design of the token it self, and how is specified through the manipulations on the tokens. 

% \jian{Specifically which step? Need to be clear here, also when talking about the process in previous subsections. Also, how do these considerations relate to the challenges before? What is the methodology employed for deriving the design considerations? }


% \jian{It is unclear how you arrived to the idea of design tokens here, then you may talk about the representation of tokes and the manipulation of tokens (D1-2 below). I wonder if this section can be better named as Design Insights. }

\subsubsection{\textbf{D2: Design tokens as a unifying concept for managing different types of design components.}}
% - how we define design token
We introduce \emph{design tokens} as the mediator between users and design elements, reifying the abstract visual information into concrete first-class graphical objects that can be directly manipulated. \jian{First, is there a need for the mediator? Can it be related to the challenges?}
This process, known as \emph{reification} \cite{beaudouin2000reification} in the instrumental interaction model \cite{beaudouin2000instrumental}, allows each visual element to become a tool in designer's hands.

% \textbf{D1.1: Types of tokens. 
% \jian{It would be great that some adjectives can be added to more precisely describe each point.}}
% - what types of tokens we consider
\textbf{D2.1: Type of tokens: managing different types of design components all through design tokens.}
We categorize design tokens into three types: \emph{visual, textual,} and \emph{imaginative}. \jian{instead of just saying "We categorize", can it be more dependent on the user insights? It is a framing thing. Generally, we avoid "we do..." in DGs because you haven't presented your solutions yet.}
Visual tokens carry visual information such as subjects, styles, and colors, primarily coming from inspirational images.
Textual tokens, complementing visual tokens, help to communicate the intent which is easier to express through language, for example, the adjective keywords to describe emotions, verb to describe gestures of a subject, or nouns to describe the surroundings.
% They complement visual tokens when the intent is better expressed through language.
Imaginative tokens mediate the initiative between designers and models. 
% This type of token resonates with designers usage of AI model: considering the AI models as a design material \cite{}.
Designers often prefer precise control over aspects like layout, colors, and the visual identity of subjects, while leveraging the model's imaginative capabilities for other details based on a specified keyword. 
For instance, one participant noted, \qt{I will leave it to the model to decide what an exact \textit{`joyful'} facial expression looks like.} 
Imaginative tokens indicate \emph{where} the model should work on and \emph{how much} imagination is needed.
    
% - why need a unifying design concept for different types of design elements
A key design insight here is that \emph{all design components should be regarded as tokens}.
The goal is not to support a complete set of all possible design components but to build an extensible paradigm with the affordance to accommodate different types. 
Such \emph{polymorphism} \cite{beaudouin2000reification} of the design tokens is essential for maintaining a simple interface with consistent interaction logic.

% \textbf{D1.2: Appearance of tokens.}
\textbf{D2.2: Appearance of tokens: trade-off between fidelity and reuse.}
The design tokens can be regarded as the abstraction depicting the design components graphically.
How to properly represent a certain component, especially visual elements, should be carefully considered.
On the one hand, design tokens must be visually distinguishable and reflect the visual information they carry. 
For example, different geometric shapes can indicate different types of visual elements, with each shape filled with the corresponding visual information. 
On the other hand, designers note that tokens should retain some degree of abstraction to suggest their potential for being re-imagined in new contexts. 
%We thus apply the style to a standard image for style tokens and attach a small screenshot of the selected subject to the corner of the subject token, rather than using the cropped image directly. 
For instance, style tokens can be represented by applying the style to a common image, and subject tokens can be represented as a small screenshot of the selected subject, instead of using the actual image cropped directly. \jian{rephrased here}

\textbf{D2.3: Life-cycle of tokens: }
To plan a design, designers often consider three aspects --- \emph{what content to construct}, \emph{how to construct it}, and \emph{in what context}.
For instance, ``two girls \emph{(content)} next to each other in the center of the image (\emph{construction way)} are dancing surrounded by flowers \emph{(context)}''.
Designers often explore alternative design possibilities by varying the construction of elements or placing them in different contexts while using the same set of visual elements. 
Therefore, tokens representing content items should be persistent for \emph{reuse} throughout the design process, while tokens describing context can be temporary for single-time use to prevent an overwhelming number of tokens from piling up in the system.

% In \sysname{}, persistent tokens are created in a separate panel and placed near their corresponding inspirational images. 
% Users can drag and drop copies of these tokens into the manipulation panel as needed. 
% Temporary tokens, on the other hand, are created and manipulated directly in the manipulation panel without creating copies. 



\subsubsection{\textbf{D3: Direct manipulation on design tokens as a natural translation of cognitive intentions to physical actions.}}
% The most noticeable tension between the designers' cognitive thoughts and expressing their intentions is xxx.
% The goal is to minimize xx.
% Long before the era of generative AI and prompt-based interfaces, HCI community has identified the pros and cons for language-medium interface and graphical interface. 
% The directness of graphical interface is widely appreciated by designers. 
% Because designers' design decisions eventually reflect on their actions; however, these actions can be hard to verbalize \cite{son2024demystifying}. 
% - why: direct manipulation is a long-standing tradition rooted in designers' workflow, particularly for quick prototyping and visual planning such as Figma: canvas as the playground to freely explore and visual planning
% - benefits: easy to learn, rapid operation, less cognitive resources (minimize cognitive efforts), direct engagement with the objects of interest

Direct manipulation \cite{hutchins1985direct} is a long-standing tradition rooted in designers' workflows, particularly for quick prototyping and visual planning. 
Tools like Figma exemplify this approach, providing a canvas as a playground for free exploration and visual planning. 
% The benefits of direct manipulation include: easy to learn, rapid operation, less cognitive efforts, and direct engagement with the objects of interest. 
In our case, users' intentions are transformed into (a series of) action specifications, and the outcomes of those actions can be translated into control signals in the model language. 

\textbf{D3.1: Intuitive and familiar actions.}
Each type of token should have intuitive actions that map directly to designers' intentions. 
For example, resizing a token should adjust its relative scale, and moving a token should specify its location. \jian{what does its refer to here?}
This intuitive mapping allows users to learn by recognizing actions rather than remembering them.
Additionally, tokens should be able to reference and influence each other. \jian{This is about tokens not actions. Does it make sense to make a new sub-point about cross-referencing actions?}
For instance, a color token can affect a subject token, or one subject token can interact with another. 
This cross-referencing enhances the expressiveness of the action vocabularies, enabling more complex design intent specifications.


\textbf{D3.2: Intermediate action outcomes.}
Designers need immediate feedback on their actions to understand how design tokens react and evaluate the outcomes of their actions. 
However, the current generative models have noticeable inference times and high computational costs, making responsive feedback for each operation impractical.
To address this, we propose a compromise. 
Instead of providing feedback for every single action, we define the granularity of feedback based on design aspects. \jian{Asepcts is very vague; what do you refer to here?}
Each design aspect is treated as a step, with feedback provided at this level of granularity. 
As the inference time of the model reduces in the future, we envision the possibilities of the on-the-fly interpretation and immediate feedback.


\textbf{D3.3: Flexible action reuse.}
Just as tokens can be reused, designers should be able to leverage their previous actions. 
Designers often revisit and explore alternative paths in their design process. 
It is necessary to support designers to easily retrace their steps, experiment with different options, and refine their work without having to repeat the actions performed.
As the actions are ultimately reflected as the construction of the design tokens, \ie, the visual lexicon, we enable the action reuse by recording each visual lexicon users have constructed. 




\jian{More literature or support may be needed for some of the above points. I feel many places are just plain arguments.}
